Context-Enhanced Vulnerability Detection Based on Large Language Model

Vulnerability detection is a critical aspect of software security. Accurate detection is essential to prevent potential security breaches and protect software systems from malicious attacks. Recently, vulnerability detection methods leveraging deep learning and large language models (LLMs) have garnered increasing attention. However, existing approaches often focus on analyzing individual files or functions, which limits their ability to gather sufficient contextual information. Analyzing entire repositories to gather context introduces significant noise and computational overhead. To address these challenges, we propose a context-enhanced vulnerability detection approach that combines program analysis with LLMs. Specifically, we use program analysis to extract contextual information at various levels of abstraction, thereby filtering out irrelevant noise. The abstracted context along with source code are provided to LLM for vulnerability detection. We investigate how different levels of contextual granularity improve LLM-based vulnerability detection performance. Our goal is to strike a balance between providing sufficient detail to accurately capture vulnerabilities and minimizing unnecessary complexity that could hinder model performance. Based on an extensive study using GPT-4, DeepSeek, and CodeLLaMA with various prompting strategies, our key findings includes: (1) incorporating abstracted context significantly enhances vulnerability detection effectiveness; (2) different models benefit from distinct levels of abstraction depending on their code understanding capabilities; and (3) capturing program behavior through program analysis for general LLM-based code analysis tasks can be a direction that requires further attention.

==> includes/0.abstract.tex <==
Vulnerability detection is crucial in the field of software security. 
Detecting vulnerabilities accurately is essential to prevent potential security breaches and protect software systems from malicious attacks. 
However, traditional approaches to vulnerability detection, which focus on analyzing individual files or functions, often fail to provide sufficient contextual information. 
On the other hand, analyzing entire repositories to gather context introduces significant noise and computational overhead.
To address these challenges, we present a context-enhanced vulnerability detection approach based on primitive API abstraction and large language models (\ie LLMs}). 
We first design a primitive API abstraction mechanism that simplifies complex function calls into fundamental API operations, thereby reducing noise while capturing critical operations related to vulnerabilities. 
The primitive API abstraction is then incorporated as contextual information in the input to the LLM, enabling the model to leverage both the natural language features of the code and the structural information captured by program analysis.
We conduct extensive empirical evaluations and the results show that compared to samples without the additional API abstraction, our method significantly improves detection performance across various types of vulnerabilities. 
%The results highlight the effectiveness of incorporating primitive API abstraction for enhancing context in vulnerability detection.
The results highlight the effectiveness of incorporating primitive API abstraction to enhance context in vulnerability detection.

==> listings/listing1.tex <==
% \begin{lstlisting}[language=C, caption={Function sg\_common\_write demonstrating a Double Free vulnerability}, label={lst:sg_common_write}]
% static int
% sg_common_write(Sg_fd * sfp, Sg_request * srp,
%                 unsigned char *cmnd, int timeout, int blocking)
% {
%     ...
%     k = sg_start_req(srp, cmnd);
%     if (k) {
%         SCSI_LOG_TIMEOUT(1, sg_printk(KERN_INFO, sfp->parentdp,
%                         "sg_common_write: start_req err=%d\n", k));
%         sg_finish_rem_req(srp);
%         return k;       /* probably out of space --> ENOMEM */
%     }
%     if (atomic_read(&sdp->detaching)) {
%         if (srp->bio)
%             blk_end_request_all(srp->rq, -EIO);
%         sg_finish_rem_req(srp);
%         return -ENODEV;
%     }
%     ...
% }
% \end{lstlisting}

\begin{lstlisting}[language=C, caption={Function sg\_common\_write demonstrating a Double Free vulnerability}, label={lst:sg_common_write}]
static int
sg_common_write(Sg_fd * sfp, Sg_request * srp,
                unsigned char *cmnd, int timeout, int blocking)
{
    ...
    k = sg_start_req(srp, cmnd);
    if (k) {
    ...
    }
    if (atomic_read(&sdp->detaching)) {
        if (srp->bio)
            blk_end_request_all(srp->rq, -EIO);
        sg_finish_rem_req(srp);
        return -ENODEV;
    }
    ...
}
\end{lstlisting}


==> listings/listing2.tex <==
\begin{lstlisting}[language=C, caption={Function sg\_finish\_rem\_req}, label={lst:sg_finish_rem_req}]
static int
sg_finish_rem_req(Sg_request *srp)
{
    int ret = 0;

    Sg_fd *sfp = srp->parentfp;
    Sg_scatter_hold *req_schp = &srp->data;

    SCSI_LOG_TIMEOUT(4, sg_printk(KERN_INFO, sfp->parentdp,
                                  "sg_finish_rem_req: res_used=%d\n",
                                  (int) srp->res_used));
    if (srp->bio)
        ret = blk_rq_unmap_user(srp->bio);

    if (srp->rq) {
        if (srp->rq->cmd != srp->rq->__cmd)
            kfree(srp->rq->cmd);
        blk_put_request(srp->rq);
    }

    if (srp->res_used)
        sg_unlink_reserve(sfp, srp);
    else
        sg_remove_scat(sfp, req_schp);

    sg_remove_request(sfp, srp);

    return ret;
}
\end{lstlisting}

==> listings/listing3.tex <==
\begin{lstlisting}[language=C, caption={Function blk\_end\_request\_all handling block request termination}, label={lst:blk_end_request_all}]
void blk_end_request_all(struct request *rq, blk_status_t error)
{
    bool pending;
    unsigned int bidi_bytes = 0;

    if (unlikely(blk_bidi_rq(rq)))
        bidi_bytes = blk_rq_bytes(rq->next_rq);

    pending = blk_end_bidi_request(rq, error, blk_rq_bytes(rq), bidi_bytes);
    BUG_ON(pending);
}
EXPORT_SYMBOL(blk_end_request_all);
\end{lstlisting}


==> tables/4.1RQ1APIBasic-1st.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for Different Primitive API Abstraction Levels with Basic Prompt}
    \vspace{2mm}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc|ccccc|ccccc}
            \hline
            & \multicolumn{5}{c|}{\textbf{GPT4o}} & \multicolumn{5}{c|}{\textbf{DeepSeek}} & \multicolumn{5}{c}{\textbf{CodeLLaMA-34b}} \\ \hline
            & {w/o} & \textbf{A1} & {A2} & {A3} & {A4} 
            & {w/o} & \textbf{A1} & \textbf{A2} & {A3} & {A4} 
            & {w/o} & {A1} & \textbf{A2} & {A3} & {A4} \\ \hline
            Accuracy & 0.47 & \textbf{0.60} & 0.54 & 0.53 & 0.54 
                     & 0.55 & \textbf{0.50} & \textbf{0.60} & 0.62 & 0.55 
                     & 0.46 & 0.43 & \textbf{0.58} & 0.47 & 0.51 \\ \hline
            Precision & 0.45 & \textbf{0.57} & 0.53 & 0.54 & 0.52 
                      & 0.48 & \textbf{0.50} & \textbf{0.53} & 0.56 & 0.47 
                      & 0.42 & 0.45 & \textbf{0.50} & 0.53 & 0.50 \\ \hline
            Recall & 0.97 & \textbf{0.80} & 0.88 & 0.78 & 0.80 
                   & 0.13 & \textbf{0.45} & \textbf{0.40} & 0.27 & 0.32 
                   & 0.20 & 0.38 & \textbf{0.81} & 0.45 & 0.46 \\ \hline
            F1 Score & 0.62 & \textbf{0.67} & 0.66 & 0.64 & 0.63 
                     & 0.21 & \textbf{0.47} & \textbf{0.46} & 0.37 & 0.38 
                     & 0.27 & 0.41 & \textbf{0.62} & 0.49 & 0.48 \\ \hline
            MCC & 0.08 & \textbf{0.22} & 0.08 & 0.02 & 0.11 
                & 0.03 & \textbf{0.00} & \textbf{0.15} & 0.16 & 0.05 
                & -0.09 & -0.13 & \textbf{0.24} & -0.05 & 0.02 \\ \hline
        \end{tabular}
    }
    \parbox{\textwidth}{\footnotesize \textit{Note}: A1–4 denotes API-Level-1–API-Level-4. W/O denotes without primitive API summaries.}

    \label{tab:basic_prompt_all_models}
\end{table}

==> tables/4.1RQ1APIBasic.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for Different Primitive API Abstraction Levels with Basic Prompt}
    \vspace{2mm}
    \renewcommand{\arraystretch}{1.5}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc|ccccc|ccccc|ccccc}
            \hline
            & \multicolumn{5}{c|}{\textbf{GPT-4o}} 
            & \multicolumn{5}{c|}{\textbf{DeepSeek-V3}} 
            & \multicolumn{5}{c|}{\textbf{DeepSeek-R1}} 
            & \multicolumn{5}{c}{\textbf{CodeLLaMA-34b}}        \\ \hline
            & {w/o} & {A1} & {A2} & {A3} & {A4} 
            & {w/o} & {A1} & {A2} & {A3} & {A4} 
            & {w/o} & {A1} & {A2} & {A3} & {A4} 
            & {w/o} & {A1} & {A2} & {A3} & {A4}                 \\ \hline
            Accuracy & 44.07 & 47.37 & 55.77 & 56.03 & 52.74
                     & 49.48 & 56.52 & 50.00 & 56.02 & 52.74
                     & 51.34 & 50.91 & 57.69 & 56.77 & 54.37
                     & 47.27 & 53.64 & 63.45 & 55.82 & 58.72    \\ \hline
            Precision & 43.84 & 44.00 & 54.87 & 56.45 & 51.03
                      & 46.15 & 50.88 & 55.00 & 55.56 & 55.56 
                      & 47.15 & 47.64 & 56.36 & 57.62 & 52.44
                      & 44.64 & 47.83 & 63.95 & 63.33 & 59.83   \\ \hline
            Recall & 93.02 & 64.71 & 77.50 & 76.64 & 69.72
                   & 83.72 & 26.13 & 13.75 & 65.48 & 14.08
                   & 83.22 & 80.80 & 77.50 & 71.31 & 69.92
                   & 75.00 & 32.35 & 71.43 & 42.54 & 50.36      \\ \hline
            F1 Score & 59.59 & 52.38 & 64.25 & 65.02 & 58.93 
                     & 59.50 & 34.52 & 22.00 & 60.11 & 22.47
                     & 60.19 & 59.94 & 65.26 & 63.74 & 59.93 
                     & 55.97 & 38.60 & 67.48 & 50.89 & 54.69    \\ \hline
            MCC & -3.96 & -2.06 & 11.63 & 10.20 & 6.76
                &  7.44 & 7.61 & 2.85 & 12.04 & 5.20
                & 11.14 & 8.06 & 15.72 & 12.11 & 9.91
                & -0.13 & 3.72 & 26.25 & 14.36 & 17.51          \\ \hline
        \end{tabular}
    }
    \parbox{\textwidth}{\footnotesize \textit{Note}: A1–4 denotes API-Level-1–API-Level-4. W/O denotes without primitive API summaries.}

    \label{tab:basic_prompt_all_models}
\end{table}

==> tables/4.2RQ1APICOT-1st.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for Different Primitive API Abstraction Levels with CoT.}
    \vspace{2mm}
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc|ccccc|ccccc}
            \hline
            & \multicolumn{5}{c|}{\textbf{GPT4o}} & \multicolumn{5}{c|}{\textbf{DeepSeek}} & \multicolumn{5}{c}{\textbf{CodeLLaMA-34b}} \\ \hline
            & w/o & \textbf{A1} & A2 & A3 & A4 & w/o & A1 & \textbf{A2} & A3 & A4 & w/o & A1 & \textbf{A2} & A3 & A4 \\ \hline
            Accuracy & 0.53 & \textbf{0.59} & 0.60 & 0.55 & 0.56 
                     & 0.49 & 0.51 & \textbf{0.60} & 0.56 & 0.55 
                     & 0.52 & 0.48 & \textbf{0.58} & 0.54 & 0.46 \\ \hline
            Precision & 0.52 & \textbf{0.55} & 0.58 & 0.56 & 0.54 
                      & 0.46 & 0.51 & \textbf{0.58} & 0.58 & 0.54 
                      & 0.37 & 0.48 & \textbf{0.50} & 0.44 & 0.42 \\ \hline
            Recall & 0.60 & \textbf{0.95} & 0.79 & 0.72 & 0.68 
                   & 0.76 & 0.75 & \textbf{0.78} & 0.66 & 0.63 
                   & 0.11 & 0.57 & \textbf{0.68} & 0.60 & 0.55 \\ \hline
            F1 Score & 0.56 & \textbf{0.70} & 0.67 & 0.63 & 0.60 
                     & 0.57 & 0.61 & \textbf{0.67} & 0.62 & 0.58 
                     & 0.17 & 0.52 & \textbf{0.58} & 0.51 & 0.48 \\ \hline
            MCC & 0.05 & \textbf{0.25} & 0.20 & 0.09 & 0.13 
                & 0.04 & 0.03 & \textbf{0.21} & 0.11 & 0.11 
                & -0.06 & -0.04 & \textbf{0.18} & 0.10 & -0.06 \\ \hline
        \end{tabular}
    }
    \parbox{\textwidth}{\footnotesize \textit{Note}: A1–4 denotes API-Level-1–API-Level-4. W/O denotes without primitive API summaries}

    \label{tab:cot_prompt_all_models}
\end{table}

==> tables/4.2RQ1APICOT.tex <==
\begin{table}[t]
    \centering
    \caption{Experimental Results for Different Primitive API Abstraction Levels with CoT.}
    \vspace{2mm}
    \renewcommand{\arraystretch}{1.4}
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccc|ccccc|ccccc|ccccc}
            \hline
            & \multicolumn{5}{c|}{\textbf{GPT-4o}} 
            & \multicolumn{5}{c|}{\textbf{DeepSeek-V3}} 
            & \multicolumn{5}{c|}{\textbf{DeepSeek-R1}} 
            & \multicolumn{5}{c}{\textbf{CodeLLaMA-34b}} \\ \hline
            & w/o & A1 & A2 & A3 & A4 
            & w/o & A1 & A2 & A3 & A4 
            & w/o & A1 & A2 & A3 & A4 
            & w/o & A1 & A2 & A3 & A4
             \\ \hline
            Accuracy & 47.94 & 44.74 & 59.62 & 55.25 & 54.45
                     & 45.23 & 47.74 & 60.90 & 54.42 & 57.79
                     & 44.25 & 44.53 & 52.29 & 53.42 & 51.33
                     & 54.38 & 54.97 & 50.00 & 46.69 & 49.83 \\ \hline
            Precision & 43.64 & 42.52 & 57.80 & 55.73 & 52.41
                      & 39.52 & 39.85 & 60.44 & 55.83 & 57.89
                      & 44.15 & 44.09 & 51.70 & 53.77 & 50.20
                      & 43.24 & 48.65 & 53.33 & 50.00 & 45.83 \\ \hline
            Recall & 59.88 & 66.91 & 78.75 & 78.10 & 69.01
                   & 46.15 & 47.32 & 68.75 & 59.82 & 54.55 
                   & 98.05 & 100.00 & 97.44 & 96.61 & 99.22
                   & 9.30  & 13.33 & 20.00 & 13.14 & 15.49 \\ \hline
            F1 Score & 50.49 & 52.00 & 66.67 & 65.05 & 59.57
                     & 42.58 & 43.27 & 64.33 & 57.76 & 56.17
                     & 60.89 & 61.20 & 67.56 & 69.09 & 66.67
                     & 15.31 & 20.93 & 20.09 & 20.81 & 23.16 \\ \hline
            MCC & -1.72 & -6.86 & 19.85 & 8.34 & 10.08
                & -9.28 & -4.57 & 21.68 & 8.41 & 15.55
                & -1.53 & 7.83 & 7.13 & -1.19 & 12.95
                & -0.71 & 2.97 & 2.00 & -2.68 & -2.64 \\ \hline
        \end{tabular}
    }
    \parbox{\textwidth}
    {\footnotesize \textit{Note}: A1–4 denotes API-Level-1–API-Level-4. W/O denotes without primitive API summaries}

    \label{tab:cot_prompt_all_models}
\end{table}
